RCM: Requirement Capturing Model for Automated Requirements Formalisation

Most existing automated requirements formalisation techniques require system engineers to (re)write their requirements using a set of predefined requirement templates with a fixed structure and known semantics to simplify the formalisation process. However, these techniques require understanding and memorising requirement templates, which are usually fixed format, limit requirements captured, and do not allow capture of more diverse requirements. To address these limitations, we need a reference model that captures key requirement details regardless of their structure, format or order. Then, using NLP techniques we can transform textual requirements into the reference model. Finally, using a suite of transformation rules we can then convert these requirements into formal notations. In this paper, we introduce the first and key step in this process, a Requirement Capturing Model (RCM) - as a reference model - to model the key elements of a system requirement regardless of their format, or order. We evaluated the robustness of the RCM model compared to 15 existing requirements representation approaches and a benchmark of 162 requirements. Our evaluation shows that RCM breakdowns support a wider range of requirements formats compared to the existing approaches. We also implemented a suite of transformation rules that transforms RCM-based requirements into temporal logic(s). In the future, we will develop NLP-based RCM extraction technique to provide end-to-end solution.

==> Formalisation.tex <==
\begin{comment}

\section{\uppercase{RCM Construction and Transformations}} \label{RCMFormalization}
\todo{In this section, we provide an overview of the NL-requirements extraction and transformation into formal notations, as shown in Fig. \ref{fig:reqFormalization}. We are working on a tool to automatically transforms NL-requirements into RCM and then into multiple formal notations. This paper only focuses on the RCM model and formal transformation. Thus, the details of the extraction algorithm utilised is out of scope.} 

\begin{figure}[htbp]
	\centering
	\includegraphics[width=\columnwidth]{rcm-paper/Crafted_Figures/PHDFlow.pdf}
	\caption{Formalizing NL-requirements}
	\label{fig:reqFormalization}
\end{figure}

\end{comment}



\subsection{Translating Natural Language Requirements to RCM}\label{construction}
%As discussed above, RCM replaces requirement boilerplates and CNL with abstract requirements capturing model. Although this solves many problems related to styling, formatting, structure of these boilerplates, it introduces a new research problem, which is how to represent requirements in RCM representation? 

%There are two options: (1) to allow system engineers to manually specify their requirements using RCM constructs (scope, trigger, action, valid-time, etc), or (2) develop automated requirements extraction technique that extract RCM components from textual requirements and construct the model automatically.  It is important to mention that this step (construction of the RCM) is outside the scope of this paper -- we mainly focus on the RCM model and transformation to formal notations. Having said that we have developed two prototypes currently under usability and soundness evaluation. The first prototype is a visual RCM modelling tool using Blockly as shown in \todo{ incliude Figure}. The second prototype is a NLP-based RCM extraction technique outlined below:  

%\todo{Do we want/need this subsection - its pretty brief - maybe just say its out of scope this paper???}

In this paper we  focus on using the RCM model to represnt safety-critical system requirements and support transformation to formal notations. However, we have developed an NLP-based tool to automatically extract the key properties of RCM from textual requirements and construct the corresponding RCM model. We outline this NLP-based RCM extraction technique below:  

%\textbf{Extraction Layer:} %in this process, the RCM is constructed. 
    \begin{itemize}
        \item \textit{Step1:} Components of a requirement sentence are identified by identifying the sentence clauses, each clause corresponds to one component.
        \item \textit{Step2:} A deep syntactic and semantic analysis are applied on each component to identify their sub-components and their breakdowns through locating and understanding the corresponding English predicate and time phrases. 
        \item \textit{Step3:} Classify requirement components and sub-components into concrete types based on semantic features (e.g., time prepositional phrases are classified to: valid-time, pre-elapsed-time, or in-between-time based on the semantic of the preposition as in Fig.\ref{fig:reqEX}).
        \item \textit{Step4:} The RCM is populated with the extraction details.
        \item \textit{Step5:} Formal semantic of Predicate and time structures are bound through matching the frame of the predicate and the relation of the time to an extendable verb-frame database that maps each frame to a unique formal semantic (e.g., the abstract frame of the predicate "if X exceeds y" is "exceed(Arg1?,Arg2?)" whose mapped formal semantic is "Arg1? $>$ Arg2?").
    \end{itemize}
    

 After Step3, each component's extractions are checked for syntactic validity (i.e., the minimal attributes of each sub component are extracted and a classification is attached). Only the passed components continue to the next steps (i.e., the others are discarded). After step4, RCMs is checked for completeness. An RCM may be populated with semantically incomplete but syntactically valid sub-component. These incompleteness issues are addressed by attaching proper artificial arguments (e.g., "After sailing termination" in Fig.\ref{fig:reqEX} is a syntactically valid NL predicate but incomplete since it has only one argument "sailing termination" thus it is corrected to "After sailing termination \ul{equals true}" with the underlined artificial arguments for completeness). After Step5, RCMs are checked for validity. RCMs with at least one action component --\emph{the mandatory component as in Fig.\ref{fig:RCMUML}}-- are flagged as Pass.

\textbf{Example RCM:}
The REQ in Fig.\ref{fig:reqEX} has two primitive requirements. PR[1] constituting of five clauses \{"After sailing termination", "if X is ON for 1 second", "Y is ON", "Z is ON", and "M shall transition to TRUE after less than 2 seconds"\}. PR[2] has three clauses \{"When the acoustical signals $<$E$>$ turns to TRUE every 1 seconds", "M shall transition to FALSE", and "before $<$B\_sig$>$ is TRUE"\}. Each clause forms one component in the corresponding RCM model. Components of each primitive requirement are presented in separate blocks in the figure. In each block, sub-components (predicate and time phrases) are separated by horizontal line. Fig.\ref{fig:reqEX} highlights the encapsulation of semi-formal semantic (in black) and formal semantic (in red). Components with the same type (e.g., conditions in PR[1]) are represented by tree structure.
%\todo{where is this figure referenced and described in the text?}

